"Global is Good, Local is Bad?": Understanding Brand Bias in LLMs

Many recent studies have investigated social biases in LLMs but brand bias has received little attention. This research examines the biases exhibited by LLMs towards different brands, a significant concern given the widespread use of LLMs in affected use cases such as product recommendation and market analysis. Biased models may perpetuate societal inequalities, unfairly favoring established global brands while marginalizing local ones. Using a curated dataset across four brand categories, we probe the behavior of LLMs in this space. We find a consistent pattern of bias in this space -- both in terms of disproportionately associating global brands with positive attributes and disproportionately recommending luxury gifts for individuals in high-income countries. We also find LLMs are subject to country-of-origin effects which may boost local brand preference in LLM outputs in specific contexts.

==> related_work.tex <==
\section{Related Work}
%\gknote{Add transition sentence here saying that we are moving on to NLP-based related work. We might consider even making related work subsections for social science and NLP.}

% Moving on to related work in NLP specifically, bias in models have been studied for word embeddings using cosine similarity (e.g., the Word Embedding Association Test) and sentence embeddings using templates such as \textit{``This will [target]''} (e.g., the Sentence Encoder Association Test.)~\cite{bolukbasi2016man,caliskan2017semantics,may2019measuring}.


% \cite{kamruzzaman2023investigating} propose a new benchmark dataset to identify social biases (ageism, beauty, institutional, and nationality) in LLMs. This motivates us to set-up our Category-1 experiment. 

% \citet{salinas2023unequal} delves into the socio-economic biases exhibited by LLMs when recommending jobs. This motivates us to set-up our Category-2 experiment. 

% Research on how LLMs favor products from certain countries, shows the impact of national biases on consumer decisions and brand loyalty (Country-of-Origin Effects) \cite{maier2017broad}. 

% As the discourse on LLM biases broadens, provides a comprehensive review of how popularity bias can skew LLM outputs, favoring popular items over less known ones \cite{klimashevskaia2023survey}.

% Lastly, \citet{winit2014global} adds a layer of complexity to the understanding of brand biases within LLMs. This paper examines the distinct preferences LLMs display towards global versus local brands, shedding light on the potential for cultural bias that could affect international marketing strategies and brand perceptions globally (Global vs. Local Brands).

% Many studies explore how marketing strategies bias consumer interactions and impact recommendation systems, advocating for a fairness-aware framework to balance market representation \citet{wan2020addressing, deldjoo2024cfairllm, ren2024survey}.

\gknote{Remove section once content has been integrated into other sections.}
%\citet{kamruzzaman2023investigating} propose a new benchmark dataset to identify social biases, including ageism, beauty, institutional, and nationality biases, in LLMs. This has motivated us to establish our Category-1 experiment.\gknote{Add a link (\texttt{\\Cref}) to the section.}
%\citet{salinas2023unequal} investigate the socio-economic biases manifested by LLMs in job recommendations. This has inspired us to initiate our Category-2 experiment.
%Research on how LLMs prefer products from specific countries demonstrates the impact of national biases on consumer decisions and brand loyalty (Country-of-Origin Effects) \cite{maier2017broad}, and this motivates us to establish our Category-3 experiment.
%As the discourse on LLM biases expands, \citet{klimashevskaia2023survey} offer a comprehensive review of how popularity bias can skew LLM outputs, favoring well-known items over lesser-known ones.
%Furthermore, \citet{winit2014global} explores the complexity and interaction effects of brand globalness.%\gknote{This is before LLMs existed. Is this a human study or a study that uses word embeddings?} 
%This study analyzes the distinct preferences people show towards global versus local brands, highlighting the potential for cultural bias that could influence international marketing strategies and brand perceptions worldwide.
%Several studies highlight how marketing strategies bias consumer interactions and affect recommendation systems. These studies advocate for a fairness-aware framework to balance market representation \cite{wan2020addressing, deldjoo2024cfairllm, ren2024survey}.
